Semantic Abstraction: Open-World 3D Scene Understanding from 2D Vision-Language Models

We study open-world 3D scene understanding, a family of tasks that require agents to reason about their 3D environment with an open-set vocabulary and out-of-domain visual inputs - a critical skill for robots to operate in the unstructured 3D world. Towards this end, we propose Semantic Abstraction (SemAbs), a framework that equips 2D Vision-Language Models (VLMs) with new 3D spatial capabilities, while maintaining their zero-shot robustness. We achieve this abstraction using relevancy maps extracted from CLIP, and learn 3D spatial and geometric reasoning skills on top of those abstractions in a semantic-agnostic manner. We demonstrate the usefulness of SemAbs on two open-world 3D scene understanding tasks: 1) completing partially observed objects and 2) localizing hidden objects from language descriptions. Experiments show that SemAbs can generalize to novel vocabulary, materials/lighting, classes, and domains (i.e., real-world scans) from training on limited 3D synthetic data. Code and data is available at https://semantic-abstraction.cs.columbia.edu/

==> tables/full_ssc.tex <==

\begin{landscape}
	\begin{table}
		\addtolength{\tabcolsep}{-4pt}
		\setlength{\tabcolsep}{0.07cm}
		\tiny
		\centering
		\input{tables/full_ssc_part1}
		\input{tables/full_ssc_part2}
		\input{tables/full_ssc_part3}
		\input{tables/full_ssc_part4}
		\input{tables/full_ssc_part5}
		\input{tables/full_ssc_part6}
		\input{tables/full_ssc_part7}
		\input{tables/full_ssc_part8}
		\caption{
			\textbf{Full OVSSC results.}
			Per-class completion performance (IoU) for all approaches. Unseen classes are shown in bold.
		}

		\label{tab:full_ssc}
	\end{table}

\end{landscape}

==> tables/full_ssc_part1.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & air conditioner & alarm clock & aluminum foil & apple & arm chair & back splash & bag  & baseball bat & baseboard & basket ball & bat & bathtub & bed  & blinds & book & bookcase & bookshelf & boots & bottle & bowl & box  & bread & bucket & burner & cabinet & can & candle & carpet & CD   & ceiling \\
	approach                          &                 &             &               &       &           &             &      &              &           &             &     &         &      &        &      &          &           &       &        &      &      &       &        &        &         &     &        &        &      &         \\
	\midrule
	SemAware                          & 47.5            & 18.3        & 0.0           & 0.5   & 48.1      & 17.7        & 0.0  & 3.1          & 33.8      & 1.0         & 0.0 & 34.9    & 65.5 & 15.3   & 4.2  & 5.5      & 4.2       & 4.9   & 6.5    & 4.8  & 3.3  & 5.1   & 0.0    & 1.4    & 31.7    & 0.0 & 1.6    & 24.0   & 4.1  & 89.9    \\
	SemAbs + \cite{chefer2021generic} & 9.4             & 1.3         & 0.0           & 1.1   & 24.5      & 6.7         & 2.9  & 1.8          & 0.6       & 1.8         & 1.1 & 10.1    & 33.6 & 7.8    & 1.0  & 18.5     & 14.2      & 0.9   & 2.8    & 1.5  & 4.7  & 4.2   & 2.3    & 1.9    & 10.3    & 0.0 & 0.3    & 5.7    & 0.4  & 50.5    \\
	Ours                              & 41.3            & 51.9        & 0.0           & 24.8  & 49.7      & 27.6        & 20.8 & 24.9         & 24.9      & 39.5        & 1.8 & 28.0    & 60.9 & 37.3   & 22.4 & 17.9     & 16.3      & 29.5  & 21.0   & 24.2 & 41.2 & 30.7  & 0.0    & 3.7    & 21.8    & 0.0 & 14.3   & 17.6   & 11.7 & 86.4    \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part2.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & ceiling fan & ceiling light & cell phone & chair & chandelier & clock & cloth & coffee machine & coffee table & collandar & column & computer & cork board & couch & counter & countertop & credit card & cup  & cup stack & curtain rod & curtains & cushion & cutting board & decal & decoration box \\
	approach                          &             &               &            &       &            &       &       &                &              &           &        &          &            &       &         &            &             &      &           &             &          &         &               &       &                \\
	\midrule
	SemAware                          & 2.9         & 5.5           & 3.8        & 31.8  & 13.1       & 0.0   & 1.8   & 7.7            & 45.9         & 0.0       & 0.0    & 5.5      & 43.8       & 53.8  & 36.2    & 28.0       & 2.2         & 6.2  & 0.0       & 13.2        & 11.0     & 34.1    & 6.9           & 8.8   & 5.4            \\
	SemAbs + \cite{chefer2021generic} & 2.7         & 5.3           & 0.7        & 11.8  & 9.7        & 1.9   & 0.8   & 8.7            & 7.8          & 0.4       & 0.0    & 2.7      & 24.9       & 27.6  & 4.1     & 8.5        & 0.3         & 1.2  & 6.8       & 2.2         & 21.8     & 8.9     & 4.0           & 3.5   & 0.0            \\
	Ours                              & 23.2        & 24.3          & 19.2       & 30.9  & 36.1       & 36.4  & 7.7   & 41.7           & 45.8         & 0.0       & 0.0    & 29.9     & 68.0       & 57.0  & 14.6    & 15.1       & 12.9        & 12.3 & 0.2       & 23.7        & 55.5     & 40.1    & 13.9          & 4.5   & 34.0           \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part3.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & decorative panel & desk & desk lamp & desktop & dining table & dish sponge & dishwasher & dog bed & dome light & door & doorknob & drawer & dresser & dumbbell & egg  & eletric plug & faucet & fireplace & floor & floor lamp & footstool & fork & fridge & garbage bag & garbage can & glass holder \\
	approach                          &                  &      &           &         &              &             &            &         &            &      &          &        &         &          &      &              &        &           &       &            &           &      &        &             &             &              \\
	\midrule
	SemAware                          & 0.0              & 31.8 & 39.6      & 2.4     & 39.5         & 0.0         & 6.4        & 0.0     & 32.4       & 50.3 & 9.2      & 20.9   & 47.5    & 0.0      & 0.0  & 0.0          & 14.9   & 42.8      & 93.9  & 38.2       & 7.6       & 1.8  & 52.6   & 38.8        & 39.7        & 0.0          \\
	SemAbs + \cite{chefer2021generic} & 0.4              & 15.4 & 8.9       & 2.2     & 13.3         & 0.6         & 15.4       & 8.0     & 8.8        & 29.9 & 1.3      & 5.5    & 20.3    & 0.5      & 0.8  & 0.0          & 2.1    & 20.6      & 12.1  & 14.6       & 6.1       & 0.4  & 22.2   & 9.7         & 7.0         & 0.0          \\
	Ours                              & 3.6              & 33.4 & 49.3      & 2.5     & 34.4         & 5.0         & 18.4       & 61.3    & 46.0       & 62.9 & 0.8      & 19.2   & 46.4    & 26.5     & 16.5 & 11.8         & 20.5   & 39.3      & 86.3  & 37.7       & 14.2      & 8.1  & 37.0   & 55.2        & 42.1        & 1.7          \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part4.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & gym weights & hand towel holder & handle & hanger & hanging ring & holding bar & house plant & jar  & kettle & key chain & keys & kitchen counter & kitchen countertop & kitchen island & kitchen vent & knife & knob & ladder & ladle & laptop & laundry hamper & lettuce & light & light fixture \\
	approach                          &             &                   &        &        &              &             &             &      &        &           &      &                 &                    &                &              &       &      &        &       &        &                &         &       &               \\
	\midrule

	SemAware                          & 0.0         & 12.2              & 17.5   & 14.6   & 0.0          & 0.0         & 14.7        & 11.9 & 3.1    & 2.6       & 2.3  & 36.9            & 24.8               & 26.9           & 0.0          & 1.6   & 14.6 & 0.3    & 3.2   & 6.5    & 24.7           & 1.2     & 5.4   & 7.8           \\
	SemAbs + \cite{chefer2021generic} & 0.7         & 1.3               & 0.0    & 0.2    & 0.0          & 4.0         & 4.2         & 2.3  & 1.5    & 0.4       & 0.5  & 13.6            & 19.5               & 14.5           & 1.6          & 0.8   & 0.6  & 17.2   & 0.8   & 3.5    & 7.4            & 2.8     & 3.7   & 5.2           \\
	Ours                              & 21.3        & 20.3              & 29.6   & 21.3   & 0.0          & 0.0         & 36.6        & 16.4 & 35.1   & 9.8       & 14.8 & 13.3            & 15.1               & 23.8           & 10.2         & 8.0   & 13.1 & 26.0   & 3.2   & 27.9   & 39.4           & 43.8    & 2.0   & 25.3          \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part5.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & light switch & loaf of sourdough & microwave & microwave platform & mirror & mobile phone & mug  & news & newspaper & novel & outlet & oven & oven hood & oven top & oven vent & painting & pan  & paper bag & paper clutter & paper towel & paper towel dispenser & paper towel roll & patio \\
	approach                          &              &                   &           &                    &        &              &      &      &           &       &        &      &           &          &           &          &      &           &               &             &                       &                  &       \\
	\midrule
	SemAware                          & 15.3         & 0.3               & 6.7       & 0.0                & 25.0   & 6.3          & 2.8  & 1.6  & 13.6      & 0.0   & 0.0    & 6.1  & 8.2       & 0.6      & 0.0       & 38.1     & 3.6  & 35.5      & 12.6          & 14.0        & 20.4                  & 3.4              & 0.0   \\

	SemAbs + \cite{chefer2021generic} & 1.6          & 4.0               & 8.3       & 4.8                & 9.9    & 0.7          & 1.0  & 0.4  & 0.3       & 0.8   & 0.1    & 16.4 & 3.3       & 1.3      & 4.5       & 16.8     & 0.9  & 2.7       & 1.3           & 0.7         & 1.7                   & 0.1              & 2.7   \\
	Ours                              & 45.2         & 34.6              & 31.6      & 0.0                & 41.2   & 10.7         & 34.5 & 10.1 & 20.3      & 4.1   & 4.9    & 21.3 & 10.4      & 1.2      & 18.3      & 61.5     & 14.7 & 23.0      & 15.7          & 9.3         & 21.3                  & 9.7              & 16.9  \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part6.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & pen  & pencil & pepper shaker & photo board & photo frame & picture frame & pillow & pipe & pitcher & plate & plunger & poster & pot  & pot lid & potato & pothos & recliner & refridgerator & remote & remote control & room decoration & rug  & safe & salt & salt shaker & scrub brush & sheet pan \\
	approach                          &      &        &               &             &             &               &        &      &         &       &         &        &      &         &        &        &          &               &        &                &                 &      &      &      &             &             &           \\
	\midrule
	Semware                           & 3.8  & 4.3    & 0.6           & 27.0        & 29.0        & 17.5          & 34.4   & 45.9 & 0.0     & 5.8   & 3.1     & 22.8   & 1.6  & 0.0     & 0.0    & 3.2    & 43.7     & 39.5          & 0.2    & 2.4            & 0.1             & 40.4 & 1.4  & 0.0  & 0.6         & 15.2        & 0.0       \\
	SemAbs + \cite{chefer2021generic} & 0.6  & 0.5    & 0.6           & 13.4        & 10.7        & 5.6           & 8.6    & 2.2  & 1.0     & 1.5   & 0.2     & 12.4   & 2.9  & 0.0     & 1.1    & 4.2    & 26.7     & 20.8          & 0.4    & 0.4            & 0.6             & 17.0 & 1.1  & 0.0  & 0.7         & 0.3         & 0.0       \\

	Ours                              & 11.9 & 7.4    & 11.1          & 44.8        & 92.7        & 30.9          & 43.7   & 17.5 & 7.8     & 18.2  & 16.9    & 48.6   & 16.3 & 0.0     & 33.9   & 32.4   & 49.6     & 35.9          & 21.4   & 22.6           & 3.4             & 41.7 & 18.1 & 0.0  & 18.7        & 12.2        & 0.0       \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part7.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & shoes & shower curtain & shower glass & shower head & side table & sink & soap bar & soap bottle & sofa & spatula & spoon & spray bottle & statue & stool & stove & sugar & sugar jar & table top decoration & teddy bear & television & tennis racket & tissue box & toaster & toilet & toilet paper \\
	approach                          &       &                &              &             &            &      &          &             &      &         &       &              &        &       &       &       &           &                      &            &            &               &            &         &        &              \\
	\midrule
	SemAware                          & 1.4   & 28.0           & 14.6         & 0.2         & 41.1       & 33.4 & 1.0      & 9.4         & 54.5 & 2.0     & 2.3   & 6.2          & 7.2    & 14.6  & 12.7  & 0.0   & 15.2      & 2.4                  & 2.5        & 27.2       & 3.7           & 4.4        & 7.0     & 50.7   & 11.9         \\
	SemAbs + \cite{chefer2021generic} & 0.6   & 8.8            & 0.7          & 0.7         & 6.7        & 11.5 & 0.3      & 1.2         & 27.4 & 1.2     & 0.4   & 1.6          & 2.0    & 3.9   & 11.1  & 1.7   & 2.7       & 0.0                  & 17.9       & 17.4       & 0.8           & 1.1        & 4.9     & 16.4   & 1.2          \\
	Ours                              & 24.4  & 40.0           & 0.3          & 11.2        & 28.7       & 27.6 & 4.1      & 33.5        & 55.4 & 3.5     & 10.3  & 43.2         & 39.5   & 17.2  & 19.4  & 2.9   & 9.9       & 0.0                  & 58.2       & 45.7       & 29.3          & 21.4       & 28.0    & 45.3   & 19.3         \\
	\bottomrule
\end{tabular}

==> tables/full_ssc_part8.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrr}
	\toprule
	{}                                & toilet paper hanger & tomato & towel & towel hanger & towel holder & towel rack & trash can & turkey pan & tv   & tv stand & vacuum cleaner & vase & wall & wardrobe & watch & water boiler & watering can & white board & window & wine bottle & wine glass & wire & workstation computer \\
	approach                          &                     &        &       &              &              &            &           &            &      &          &                &      &      &          &       &              &              &             &        &             &            &      &                      \\
	\midrule
	SemAware                          & 14.5                & 2.5    & 0.0   & 0.0          & 12.1         & 0.0        & 41.0      & 0.0        & 26.5 & 41.9     & 43.1           & 10.4 & 66.6 & 11.0     & 0.9   & 0.0          & 2.9          & 38.9        & 30.2   & 4.5         & 3.8        & 14.3 & 2.4                  \\
	SemAbs + \cite{chefer2021generic} & 0.5                 & 2.0    & 0.9   & 0.4          & 2.2          & 0.0        & 9.3       & 1.3        & 17.6 & 11.4     & 4.4            & 1.6  & 14.2 & 6.3      & 0.3   & 0.6          & 0.6          & 43.9        & 16.7   & 5.6         & 4.3        & 1.0  & 3.4                  \\
	Ours                              & 11.7                & 27.1   & 7.8   & 0.4          & 13.8         & 0.0        & 47.1      & 1.6        & 46.6 & 22.6     & 35.9           & 25.0 & 61.3 & 21.1     & 12.8  & 25.2         & 17.5         & 85.8        & 40.4   & 41.8        & 13.1       & 13.7 & 2.9                  \\
	\bottomrule
\end{tabular}

==> tables/sscv1.tex <==
\begin{table*}[t]
	\addtolength{\tabcolsep}{-3pt}
	%   \footnotesize
	\centering
	\begin{tabular}{l@{\hskip -0.1cm}c@{\hskip -0.1cm}ccccccc}
		\toprule
		\multirow{2}{2cm}{\hfill Approach}      & \textbf{Unseen Instances} & \multicolumn{6}{c}{\textbf{Unseen Classes}}                                                                                 \\\cmidrule(lr){2-2}\cmidrule(lr){3-8}
		                                        & average                   & clock                                       & piano         & dumbbell      & basketball    & teddy bear    & average       \\\midrule
		No SemAbs                               & 24.3                      & 0.0                                         & 1.6           & 0.0           & 0.3           & 2.0           & XX.X          \\
		SemAbs + \citeauthor{chefer2021generic} & 16.5                      & 5.0                                         & \textbf{22.9} & 0.4           & 4.4           & 22.1          & XX.X          \\
		\midrule
		Ours                                    & \textbf{28.4}             & \textbf{26.9}                               & 19.4          & \textbf{12.7} & \textbf{32.7} & \textbf{41.4} & \textbf{XX.X} \\
		\bottomrule
	\end{tabular}
	\caption{
		\centering
		\textbf{Open Vocabulary Semantic Scene Completion.}
		TODO: consider calling Unseen Instances in distribution.
	}
	\label{tab:ovssc}
\end{table*}

==> tables/sscv2.tex <==
\begin{table*}[t]
	\addtolength{\tabcolsep}{-3pt}
	%   \footnotesize
	\centering
	\begin{tabular}{lccccccccc}
		\toprule
		\multirow{2}{2cm}
		\hfill Approach
		          & \textbf{ID}
		          & \textbf{OOD V}
		          & \textbf{OOD L}
		          & \multicolumn{5}{c}{\textbf{OOD V+L}}                                                                      \\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-10}
		          &                                      &  &  & clock & piano & dumbbell & basketball & teddy bear & average \\\midrule
		No SemAbs & 24.3                                 &  &  & 0.0   & 1.6   & 0.0      & 0.3        & 2.0        & XX.X    \\
		% SemAbs + \citeauthor{chefer2021generic} & 16.5          & 5.0            & \textbf{22.9}  & 0.4                                  & 4.4           & 22.1          & XX.X          \\
		% \midrule
		% Ours                                    & \textbf{28.4} & \textbf{26.9}  & 19.4           & \textbf{12.7}                        & \textbf{32.7} & \textbf{41.4} & \textbf{XX.X} \\
		\bottomrule
	\end{tabular}
	\caption{
		\centering
		\textbf{Open Vocabulary Semantic Scene Completion.}
		TODO: consider calling Unseen Instances in distribution.
	}
	\label{tab:ovssc}
\end{table*}

==> tables/sscv3.tex <==
\begin{table*}[t]
	\addtolength{\tabcolsep}{-4pt}
	\footnotesize
	\centering
	\begin{tabular}{l@{\hskip -0.1cm}cccccccc}
		\toprule
		\multirow{2}{1cm}{\hfill Approach} & \textbf{UnScenes} & \textbf{UnVoc} & \multicolumn{5}{c}{\textbf{UnCla}}                                                                 \\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-8}
		                                   & avg               & name           & clock                              & piano         & dumbbell      & basketball    & teddy bear    \\\midrule
		SemAware                           & 24.3              &                & 0.0                                & 1.6           & 0.0           & 0.3           & 2.0           \\
		SemAbs+\cite{chefer2021generic}    & 16.5              &                & 5.0                                & \textbf{22.9} & 0.4           & 4.4           & 22.1          \\
		\midrule
		Ours                               & \textbf{28.4}     &                & \textbf{26.9}                      & 19.4          & \textbf{12.7} & \textbf{32.7} & \textbf{41.4} \\
		\bottomrule
	\end{tabular}
	\caption{
		\centering
		\textbf{Open Vocabulary Semantic Scene Completion.}
	}
	\label{tab:ovssc}
\end{table*}

==> tables/voolv1.tex <==
\begin{table*}[t]
	% \addtolength{\tabcolsep}{-3pt}
	% \footnotesize
	\centering
	\begin{tabular}{lcccccc}
		\toprule
		\multirow{2}{2.4cm}{\hfill Approach}    & \textbf{Unseen Instances} & \multicolumn{5}{c}{\textbf{Unseen Attributes}}                                                                 \\\cmidrule(lr){2-2}\cmidrule(lr){3-7}
		                                        & average                   & name                                           & color         & material      & class         & average       \\\midrule
		No SemAbs                               & XX.X                      & XX.X                                           & XX.X          & XX.X          & XX.X          & XX.X          \\
		SemAbs + \citeauthor{chefer2021generic} & XX.X                      & XX.X                                           & XX.X          & XX.X          & XX.X          & XX.X          \\
		ClipSpatial                             & XX.X                      & XX.X                                           & XX.X          & XX.X          & XX.X          & XX.X          \\
		\midrule
		Ours                                    & \textbf{XX.X}             & \textbf{XX.X}                                  & \textbf{XX.X} & \textbf{XX.X} & \textbf{XX.X} & \textbf{XX.X} \\
		\bottomrule
	\end{tabular}
	\caption{
		% \centering
		\textbf{Visible \& Hidden Object Localization.}
		After training on a distribution of classes, colors, and materials (\eg wooden chair, red box), we test on language inputs which are in-distribution (\textbf{Unseen instances}) and out-of-distribution (\textbf{Unseen Attributes}) which refers to novel classes, colors, and materials (\eg, leather recliner, purple box).
		TODO: Also consider novel names? (OOD language only).
	}
	\label{tab:vool}
\end{table*}

==> tables/voolv2.tex <==

\begin{wraptable}{r}{0.52\textwidth}
	\vspace{-6mm}
	\setlength{\tabcolsep}{0.09cm}
	\footnotesize
	\centering
	\begin{tabular}{lcccc}
		\toprule
		\multirow{2}{1cm}{\hfill Approach} & \textbf{UnScene} & \multicolumn{2}{c}{\textbf{UnVoc}} & \textbf{UnCla}       \\
		\cmidrule(lr){2-2}\cmidrule(lr){3-4}\cmidrule(lr){5-5}
		                                   & name             & name                               & material       & avg \\\midrule
		SemAware                           & XX.X             & XX.X                               & XX.X           &     \\
		SemAbs + \cite{chefer2021generic}  & XX.X             & XX.X                               & XX.X           &     \\
		ClipSpatial                        & XX.X             & XX.X                               & XX.X           &     \\
		\midrule
		Ours                               & \textbf{XX.X}    & \textbf{XX.X}                      & \textbf{XX.X}  & X   \\
		\bottomrule
	\end{tabular}
	\vspace{-1mm}
	\caption{\textbf{Visually Obscured Object Localization}}
	\label{tab:vool}
	\vspace{-6mm}
\end{wraptable}

==> text/full_nyu_perclass.tex <==
\subsection{NYUCAD Zero-shot SSC performance breakdown by object category}
\label{sec:nyucad_full_list}
\begin{multicols}{3}
	\begin{itemize}\setlength\itemsep{0.05em}
		\footnotesize
		\item briefcase : 72.0
		\item grandfather clock : 67.2
		\item cat : 65.3
		\item cat cage : 62.8
		\item baby chair : 61.3
		\item bicycle : 59.2
		\item bag of bagels : 57.6
		\item jacket : 53.7
		\item cart : 51.3
		\item globe : 50.4
		\item bed : 50.0
		\item fax machine : 47.7
		\item dresser : 47.0
		\item basketball hoop : 46.9
		\item electrical kettle : 45.0
		\item floor : 44.8
		\item garbage bag : 39.4
		\item key : nan
		\item pool table : 78.1
		\item paper towel dispenser : 73.3
		\item tent : 69.3
		\item projector : 68.3
		\item playpen : 67.1
		\item luggage : 66.1
		\item papers : 64.0
		\item tuna cans : 62.7
		\item pizza box : 57.9
		\item piano : 56.0
		\item toilet : 54.7
		\item plastic crate : 54.0
		\item radiator : 53.6
		\item paper cutter : 50.6
		\item salt and pepper : 50.0
		\item treadmill : 49.6
		\item sofa : 48.9
		\item toys rack : 46.4
		\item wardrobe : 45.2
		\item ladder : 44.7
		\item suitcase : 42.8
		\item flower : 42.5
		\item dog bowl : 42.2
		\item football : 40.9
		\item column : 40.8
		\item stroller : 40.8
		\item table runner : 40.3
		\item map : 40.1
		\item plastic dish : 39.5
		\item plant : 39.5
		\item napkin holder : 39.4
		\item curtain : 39.1
		\item chandelier : 38.9
		\item bunk bed : 38.6
		\item television : 38.2
		\item water purifier : 38.2
		\item whiteboard : 38.0
		\item cabinet : 37.8
		\item night stand : 37.6
		\item step stool : 37.4
		\item chart stand : 36.5
		\item corkscrew : 36.4
		\item fish tank : 35.6
		\item garage door : 35.5
		\item laptop : 35.2
		\item blinds : 35.2
		\item package of bottled water : 34.2
		\item toaster oven : 34.2
		\item wall : 33.7
		\item laundry basket : 33.5
		\item stuffed animal : 33.4
		\item toiletries bag : 33.3
		\item wine bottle : 33.3
		\item toy stroller : 33.1
		\item lamp : 32.8
		\item backpack : 32.8
		\item toy kitchen : 32.3
		\item poster board : 32.2
		\item shower curtain : 32.2
		\item refridgerator : 32.2
		\item hand sculpture : 32.1
		\item yoga mat : 31.9
		\item printer : 31.8
		\item bathtub : 31.8
		\item ironing board : 31.7
		\item toyhouse : 31.3
		\item water heater : 31.2
		\item crate : 30.7
		\item pineapple : 30.6
		\item counter : 30.4
		\item fire extinguisher : 30.2
		\item monitor : 30.1
		\item garbage bin : 29.9
		\item ceiling : 29.8
		\item coffee table : 29.8
		\item ornamental item : 29.6
		\item mirror : 29.4
		\item window : 29.1
		\item hockey stick : 28.9
		\item bread : 28.6
		\item headboard : 28.4
		\item bookshelf : 27.9
		\item spice rack : 27.8
		\item pyramid : 27.7
		\item manilla envelope : 27.5
		\item blender : 27.5
		\item urn : 27.4
		\item music keyboard : 27.2
		\item oven : 27.2
		\item kitchen container plastic : 26.9
		\item basket : 26.7
		\item fan : 26.6
		\item humidifier : 26.5
		\item guitar : 26.2
		\item display board : 26.0
		\item door : 25.5
		\item microwave : 25.3
		\item face wash cream : 25.0
		\item file pad : 25.0
		\item glass ware : 25.0
		\item kitchen island : 25.0
		\item decorative bowl : 24.8
		\item fireplace : 24.3
		\item pillow : 24.2
		\item bucket : 24.1
		\item clothing drying rack : 24.1
		\item dog : 24.1
		\item tv stand : 24.0
		\item desk : 23.9
		\item vase : 23.6
		\item xbox : 23.5
		\item bag of hot dog buns : 23.4
		\item stairs : 23.3
		\item shorts : 23.1
		\item bench : 22.8
		\item rolled carpet : 22.3
		\item doll : 22.2
		\item pot : 22.1
		\item plaque : 21.9
		\item certificate : 21.7
		\item stove burner : 21.4
		\item air conditioner : 21.2
		\item contact lens solution bottle : 20.9
		\item clothes : 20.8
		\item crock pot : 20.5
		\item furniture : 20.5
		\item cd : 20.4
		\item crib : 20.4
		\item cork board : 20.4
		\item tissue box : 20.3
		\item tea pot : 20.3
		\item machine : 20.3
		\item stool : 20.3
		\item table : 20.1
		\item books : 20.1
		\item decorative dish : 20.0
		\item blanket : 19.9
		\item stereo : 19.9
		\item picture : 19.9
		\item hat : 19.6
		\item kitchen items : 19.6
		\item music stereo : 19.5
		\item shelves : 19.5
		\item stove : 19.4
		\item coffee machine : 19.3
		\item calendar : 19.2
		\item plant pot : 19.1
		\item chair : 19.0
		\item water carboy : 18.8
		\item pitcher : 18.7
		\item bookend : 18.4
		\item door knob : 18.2
		\item sponge : 18.0
		\item window shelf : 17.9
		\item cat bed : 17.9
		\item paper towel : 17.2
		\item hamburger bun : 17.1
		\item album : 16.9
		\item shoe : 16.7
		\item hookah : 16.1
		\item tea kettle : 16.0
		\item bottle : 15.9
		\item file : 15.7
		\item notebook : 15.7
		\item toaster : 15.7
		\item menorah : 15.7
		\item computer : 15.7
		\item purse : 15.5
		\item serving dish : 15.2
		\item electric toothbrush : 15.0
		\item bowl : 15.0
		\item toilet paper : 15.0
		\item chessboard : 14.8
		\item sink : 14.7
		\item towel : 14.7
		\item dvd player : 14.6
		\item piano bench : 14.6
		\item cable box : 14.6
		\item collander : 14.4
		\item clock : 14.3
		\item floor mat : 14.2
		\item toy house : 14.1
		\item speaker : 14.0
		\item drawer : 13.8
		\item foot rest : 13.7
		\item magazine : 13.7
		\item banana : 13.7
		\item room divider : 13.7
		\item dvds : 13.6
		\item flower pot : 13.5
		\item trophy : 13.3
		\item heating tray : 13.3
		\item candlestick : 12.8
		\item frying pan : 12.7
		\item mantel : 12.4
		\item puppy toy : 12.4
		\item box : 12.3
		\item wall stand : 12.3
		\item decorative platter : 12.2
		\item bag of chips : 12.2
		\item can : 12.1
		\item copper vessel : 12.0
		\item alarm clock : 11.8
		\item faucet : 11.6
		\item baking dish : 11.5
		\item board : 11.5
		\item banister : 11.5
		\item pencil : 11.5
		\item glass baking dish : 11.2
		\item stapler : 11.0
		\item bag : 11.0
		\item heater : 10.7
		\item sock : 10.4
		\item ottoman : 10.2
		\item paper : 10.2
		\item tennis racket : 10.1
		\item cup : 10.1
		\item fruit stand : 9.8
		\item sheets : 9.8
		\item apple : 9.8
		\item dishwasher : 9.7
		\item music stand : 9.6
		\item container : 9.5
		\item rug : 9.5
		\item drying rack : 9.4
		\item basketball : 9.3
		\item wire : 9.2
		\item book : 9.0
		\item soap : 8.9
		\item placemat : 8.9
		\item guitar case : 8.9
		\item electronic drumset : 8.7
		\item toy truck : 8.6
		\item person : 8.4
		\item tray : 8.3
		\item glass container : 8.0
		\item light : 7.9
		\item keyboard : 7.8
		\item range hood : 7.7
		\item router : 7.5
		\item vessel : 7.4
		\item folder : 7.4
		\item bagel : 7.4
		\item toy box : 7.0
		\item wall decoration : 6.8
		\item toy boat : 6.8
		\item sink protector : 6.7
		\item drying stand : 6.7
		\item jar : 6.7
		\item ipod : 6.7
		\item thermostat : 6.4
		\item pen : 6.3
		\item decoration item : 6.2
		\item toy : 6.1
		\item hair brush : 6.1
		\item glass dish : 5.9
		\item sculpture : 5.9
		\item exit sign : 5.8
		\item electrical outlet : 5.7
		\item sleeping bag : 5.7
		\item magnet : 5.4
		\item classroom board : 5.3
		\item vacuum cleaner : 5.2
		\item cutting board : 5.1
		\item napkin : 5.1
		\item pipe : 4.9
		\item bin : 4.5
		\item hand sanitizer dispenser : 4.5
		\item plate : 4.4
		\item pen box : 4.3
		\item pen stand : 4.2
		\item deoderant : 4.2
		\item duster : 4.1
		\item tape dispenser : 4.0
		\item canister : 4.0
		\item mask : 3.7
		\item air vent : 3.6
		\item scarf : 3.6
		\item telephone : 3.3
		\item toy cash register : 3.2
		\item scale : 3.2
		\item game system : 3.2
		\item envelopes : 3.1
		\item brick : 3.1
		\item webcam : 3.0
		\item light switch : 2.9
		\item cell phone : 2.9
		\item poster case : 2.3
		\item remote control : 2.2
		\item medal : 2.1
		\item mattress : 2.1
		\item towel rod : 2.0
		\item candle : 1.9
		\item cannister : 1.8
		\item water dispenser : 1.5
		\item button : 1.4
		\item knife rack : 1.2
		\item steamer : 1.1
		\item shaver : 0.9
		\item file box : 0.9
		\item faucet handle : 0.8
		\item radio : 0.8
		\item toy car : 0.8
		\item eraser : 0.7
		\item magazine holder : 0.5
		\item mug holder : 0.4
		\item unknown : 0.0
		\item baby gate : 0.0
		\item banana peel : 0.0
		\item bar of soap : 0.0
		\item belt : 0.0
		\item binder : 0.0
		\item book holder : 0.0
		\item bottle of perfume : 0.0
		\item broom : 0.0
		\item bulb : 0.0
		\item cap stand : 0.0
		\item case : 0.0
		\item celery : 0.0
		\item cell phone charger : 0.0
		\item chart : 0.0
		\item chimney : 0.0
		\item circuit breaker box : 0.0
		\item clothing hanger : 0.0
		\item comb : 0.0
		\item comforter : 0.0
		\item console system : 0.0
		\item corn : 0.0
		\item decorative item : 0.0
		\item decorative plate : 0.0
		\item desk mat : 0.0
		\item dish brush : 0.0
		\item dog cage : 0.0
		\item drum : 0.0
		\item dvd : 0.0
		\item eggs : 0.0
		\item ethernet jack : 0.0
		\item filing shelves : 0.0
		\item flag : 0.0
		\item flipboard : 0.0
		\item gift wrapping : 0.0
		\item glass : 0.0
		\item glass pot : 0.0
		\item grill : 0.0
		\item hole puncher : 0.0
		\item hot dogs : 0.0
		\item ipod dock : 0.0
		\item jeans : 0.0
		\item jug : 0.0
		\item juicer : 0.0
		\item kichen towel : 0.0
		\item kinect : 0.0
		\item knife : 0.0
		\item lid : 0.0
		\item lunch bag : 0.0
		\item mail tray : 0.0
		\item microphone : 0.0
		\item mouse : 0.0
		\item mug hanger : 0.0
		\item notecards : 0.0
		\item orange juicer : 0.0
		\item orange plastic cap : 0.0
		\item pan : 0.0
		\item pen holder : 0.0
		\item phone jack : 0.0
		\item plastic tray : 0.0
		\item projector screen : 0.0
		\item quilt : 0.0
		\item ruler : 0.0
		\item sculpture of the chrysler building : 0.0
		\item sculpture of the eiffel tower : 0.0
		\item sculpture of the empire state building : 0.0
		\item serving spoon : 0.0
		\item sheet music : 0.0
		\item shoe hanger : 0.0
		\item shofar : 0.0
		\item show piece : 0.0
		\item shower cap : 0.0
		\item sign : 0.0
		\item slide : 0.0
		\item spatula : 0.0
		\item spoon stand : 0.0
		\item squeeze tube : 0.0
		\item stand : 0.0
		\item suger jar : 0.0
		\item toy apple : 0.0
		\item toy horse : 0.0
		\item toys basket : 0.0
		\item trivet : 0.0
		\item vegetable : 0.0
		\item vegetable peeler : 0.0
		\item vegetables : 0.0
		\item vessel set : 0.0
		\item video game : 0.0
		\item wall hand sanitizer dispenser : 0.0
		\item water filter : 0.0
		\item watermellon : 0.0
		\item whisk : 0.0
		\item whiteboard marker : 0.0
		\item window box : 0.0
		\item window seat : 0.0
		\item wine accessory : 0.0
		\item wire rack : 0.0
		\item wooden container : 0.0
		\item wooden plank : 0.0
		\item yarmulka : 0.0
	\end{itemize}
\end{multicols}

==> text/rebuttal.tex <==
{
\color{blue}
\section{Additional Experiments in Discussion Period}

%NYUCAD is a standard closed-world SSC benchmark, which uses posed RGB images from the NYUv2 dataset~\cite{silberman2012indoor} and CAD-based 3D ground truths~\cite{guo2015predicting}.
% \textbf{Data Preprocessing.}
% We modified the
% \href{https://github.com/shurans/sscnet/blob/master/matlab_code/perpareNYUCADdata.m}{voxelization code}
% from
% \citeauthor{song2017semantic}
% to output a ground truth voxel of dimensions $480\times 480\times 244$ over the full list of 894 categories.
% This ground truth volume is used to subsample query points from during our training.
% Further, we rotate the scene along the Z axis to align the camera viewing orientation (\ie azimuth) with the positive Y axis.

% \textbf{Training.}
% We follow the same training procedure and use the same network architecture (\ie 3D UNet backbone~\cite{abdulkadir2016unet3d} with 5 levels for $f_{encode}$ and a two layer MLP for $f_{decode}$) as we did for our OVSSC task (\S~\ref{sec:method:ovssc}).
% Namely, in each batch, we sample $B$ scenes, $K$ object categories within each scene, and subsample $N$ points from each category's relevancy point cloud as input to our module.
% Similar to our OVSSC training, we apply small random transformations on the input and query points, and optimize the predicted occupancy log probability point clouds to their ground truth occupancy using binary cross entropy (BCE).
% We use balance sampling to subsample $M$ query points from the ground truth volume to balance between positive and negative labels.
% For scenes with less than $K$ object categories, we pad the remaining dimensions with zeros and do not supervise their loss.
% The network is optimized with the cosine learning rate scheduler with restarts, AdamW optimizer with $1e-4$ weight decay, $1e-4$ learning rate, $256$ warmup steps, batch size $B = 8$, $K = 12$, number of input points $N = 50000$, number of output points $M = 50000$.

%\textbf{Evaluation.}

\subsection{Comparison to Visual Grounding Method}

We include quantitative comparison with LAVT~\cite{yang2022lavt} (Tab.~\ref{tab:vool}), a state of the art (SOTA) VLM for referring expression segmentation on the RefCOCO+ benchmark~\cite{yu2016modeling}, in our VOOL task.
Since LAVT is only capable of outputting 2D segmentations of expressions, we use its segmentation masks~\footnote{
	We directly use the demo inference script provided by \href{https://github.com/yz93/lavt-ris}{https://github.com/yz93/lavt-ris}.
	The masks which the script outputs are used as input to LAVTSpatial's 3D network.
} as input to our 3D network.
We refer to this baseline as LAVTSpatial.
Similar to the CLIPSpatial baseline (discussed in \S~\ref{sec:eval}), LAVTSpatial offloads both semantic and spatial reasoning to the 2D VLM, and only learns to map partial pointclouds to completed 3D occupancies.

Quantatively, LAVTSpatial achieves the worse performance out of all variations (fourth row, Tab.~\ref{tab:vool}), at less than 2.5 IoU across all generalization scenarios.
We hypothesize that LAVT's significantly smaller and less diverse training data (\ie RefCOCO+, 150 thousand expressions) compared to CLIP's (\ie 400 million image-pairs) leads to a less robust zeroshot visual encoder.
Qualitatively (Fig.~\ref{fig:lavt_comparison}), we observe that while LAVT can sometimes propose object masks which has a better matching with object boundaries compared to our relevancy maps, these masks are rarely on the referred object.
In both cases, the 2D VLMs fail to exhibit 3D spatial understanding.
For instance, CLIP's relevancy maps for "harry potter book in the book shelf" and "rapid test behind the harry potter book" are very similar.
In other cases, both the reference and target objects are highlighted (\eg "plant on top of the book shelf", "light switch to the left of the door").
These results further support our claim in \S~\ref{sec:eval}, that while CLIP relevancy is useful for detecting objects, we should not rely on it for spatial understanding.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/lavt_comparison.png}
	\caption{
		\color{blue}
		\textbf{Comparison to LAVT.}
		For our relevancy extractor, we visualize the raw relevancy values using the jet color map.
		For LAVT, we visualize its mask in red. Quantities evaluation shown in Tab. \ref{tab:vool}.
	}
	\label{fig:lavt_comparison}
\end{figure}



}


